Well-Read Students Learn Better: On the Importance of Pre-training Compact Models

Recent developments in natural language representations have been accompanied by large and expensive models that leverage vast amounts of general-domain text through self-supervised pre-training. Due to the cost of applying such models to down-stream tasks, several model compression techniques on pre-trained language representations have been proposed (Sun et al., 2019; Sanh, 2019). However, surprisingly, the simple baseline of just pre-training and fine-tuning compact models has been overlooked. In this paper, we first show that pre-training remains important in the context of smaller architectures, and fine-tuning pre-trained compact models can be competitive to more elaborate methods proposed in concurrent work. Starting with pre-trained compact models, we then explore transferring task knowledge from large fine-tuned models through standard knowledge distillation. The resulting simple, yet effective and general algorithm, Pre-trained Distillation, brings further improvements. Through extensive experiments, we more generally explore the interaction between pre-training and distillation under two variables that have been under-studied: model size and properties of unlabeled task data. One surprising observation is that they have a compound effect even when sequentially applied on the same data. To accelerate future research, we will make our 24 pre-trained miniature BERT models publicly available.

==> figures/pd_algorithm.tex <==
\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{algorithm}[t]
%\scalebox{.85}{
    \begin{algorithmic}[1]
        \Require {
            %\footnotesize 
            student $\theta$, teacher $\Omega$,
            unlabeled LM data $\D_{LM}$, unlabeled transfer data $\D_{T}$, labeled data $\D_{L}$
        }
        \vspace{2mm}
        \State Initialize $\theta$ by pre-training an MLM$^+$ on $\D_{LM}$
       \ForEach {$x \in \D_T$}
       \State Get loss $L \gets -\sum_{y} P_\Omega(y | x) \log P_\theta(y | x)$
       \State Update student $\theta \gets \textsc{backprop}(L, \theta)$
       \eat{
        \For{$n \gets 1$ to $\textsc{distillation}\_\textsc{steps}$}
            \State Sample a batch  $x^1,x^2,\ldots x^k$ from $\D_T$
            \State Obtain soft labels from the teacher:
            \vspace{-2mm}
            \[q^i=P_\Omega(x^i), \forall i=1\ldots k\]
            \State Update $\theta$ by minimizing cross-entropy: 
            \vspace{-2mm}
            \[ -\frac{\partial }{\partial \theta}(\sum_{i=1}^k {\E}_{q^i} [-\log P_\theta(x^i)])\]
            }
        \EndFor
        \State Fine-tune $\theta$ on $\D_L$ \Comment{Optional step.}
        \State \Return $\theta$
    \end{algorithmic}
    %}
    \caption{\recipename} \label{algo:receipe}
\end{algorithm}

==> figures/tiny_results.tex <==
\begin{table}[]
    \vspace{-10pt}
    \centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{l|l|g|c|c|c|c|c|c}
         \toprule
         & Model & Meta & SST-2 & MRPC & QQP & MNLI & QNLI & RTE \\
         & 
            & Score 
            & \footnotesize (acc)
            & \footnotesize (f1/acc)
            & \footnotesize (f1/acc)
            & \footnotesize (acc m/mm)
            & \footnotesize (acc)
            & \footnotesize (acc) \\
         \midrule
         \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{test}}}
         & PF &
            TODO &      % Score
            TODO &      % SST-2
            TODO &      % MRPC
            TODO &      % QQP
            TODO &      % MNLI
            TODO &      % QNLI
            TODO \\     % RTE
         & PD &
            74.1 &              % Score
            83.5 &              % SST-2
            80.8/71.2 &         % MRPC
            63.0/84.0 &         % QQP
            72.9/72.6 &         % MNLI
            79.8 &              % QNLI
            59.1 \\             % RTE
         & PD$^+$F &
            TODO &      % Score
            TODO &      % SST-2
            TODO &      % MRPC
            TODO &      % QQP
            TODO &      % MNLI
            TODO &      % QNLI
            TODO \\     % RTE
         \midrule
         \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{dev}}}
         & PF &
            TODO &              % Score
            81.8 &              % SST-2
            81.5/71.3 &         % MRPC
            81.7/85.6 &         % QQP
            TODO &      % MNLI
            78.5 &              % QNLI
            59.1 \\             % RTE
         & PD &
            75.9 &              % Score
            81.7 &              % SST-2
            82.4/73.0 &         % MRPC
            82.3/86.2 &         % QQP
            72.7/73.2 &         % MNLI
            79.2 &              % QNLI
            59.1 \\             % RTE
         & PD$^+$F &
            TODO &      % Score
            TODO &      % SST-2
            TODO &      % MRPC
            TODO &      % QQP
            TODO &      % MNLI
            TODO &      % QNLI
            TODO \\     % RTE
         \bottomrule
    \end{tabular}
    %} % end \resizebox
    % A tabular is "fragile command" in a "moving argument". See https://texfaq.org/FAQ-extrabrace.
    \caption[sanitization argument]{
        \textbf{Baselines for future work}:\vspace{2mm}
        \small
        \begin{tabular}{ll}
            PF: & \PtFt \\
            PD: & Pre-trained Distillation on \DT$=$\DL \\
            PD$^+$F: & Pre-trained Distillation on \DT$>$\DL, fine-tuned on \DL \\
        \end{tabular}
        All students are 2L/128H BERT models, trained by 12L/768H BERT teachers. For PD and PD$^+$F, softmax temperature was set to 100. Hyperparameter sweeps include: batch size (32, 64, 128), learning rate (2e-05, 5e-05) and training epochs (3, 4, 10). Dev results are averaged over 5 runs with different seeds for the best hyperparameter setting. Test results are evaluated on the GLUE server, using the model that performed best on dev. The meta score is computed on 6 tasks only, and it is \underline{not} directly comparable to the GLUE leaderboard.
    }
    \label{tab:tiny_results}
    \vspace{-10pt}
\end{table}
